Graph Theory and its Uses in Graph Algorithms and Beyond

Graphs are fundamental objects that find widespread applications across computer science and beyond. Graph Theory has yielded deep insights about structural properties of various families of graphs, which are leveraged in the design and analysis of algorithms for graph optimization problems and other computational optimization problems. These insights have also proved helpful in understanding the limits of efficient computation by providing constructions of hard problem instances. At the same time, algorithmic tools and techniques provide a fresh perspective on graph theoretic problems, often leading to novel discoveries. In this thesis, we exploit this symbiotic relationship between graph theory and algorithms for graph optimization problems and beyond. This thesis consists of three parts. In the first part, we study a graph routing problem called the Node-Disjoint Paths (NDP) problem. Given a graph and a set of source-destination pairs of its vertices, the goal is to route the maximum number of pairs via node-disjoint paths. We come close to resolving the approximability of NDP by showing that it is $n^{\Omega(1/poly\log\log n)}$-hard to approximate, even on grid graphs, where n is the number of vertices. In the second part of this thesis, we use graph decomposition techniques developed for efficient algorithms to derive a graph theoretic result. We show that for every n-vertex expander graph G, if H is any graph with at most $O(n/\log n)$ vertices and edges, then H is a minor of G. In the last part, we show that the graph theoretic tools and graph algorithmic techniques can shed light on problems seemingly unrelated to graphs. We show that the randomized space complexity of the Longest Increasing Subsequence (LIS) problem in the streaming model is intrinsically tied to the query-complexity of the Non-Crossing Matching problem on graphs in a new model of computation that we define.

==> abstract.tex <==
\input{stdio}

\begin{document}

\title{
    On Graph Routing, Graph Minors, and Non-Crossing Matchings\\
    \vspace{0.7em}
    \Large Thesis Proposal} 
\author{Rachit Nimavat}
\maketitle

\thispagestyle{empty}
\begin{abstract}
    \input{long_abstract}
\end{abstract}


\end{document}


==> ncm/abstract.tex <==
We initiate the study of the query complexity of estimating the size of a largest {\em non-crossing matching} (\NCM)  in a bipartite graph.
Given a bipartite graph $G(L , R, E)$ with ordered vertex sets $L$ and $R$, a matching $M$ in $G$ is \emph{non-crossing} if, for every pair of edges $(u,v), (u', v') \in M$, if $u < u'$, then $v < v'$ holds.
One of our primary motivations for studying the {\em query complexity} of \NCM estimation is its intimate connection to the {\em space complexity} of the extensively studied longest increasing subsequence (\LIS) problem in the streaming model of computation.
It is known that \LIS length can be approximated to within an $O(1)$ factor in $O(\sqrt{N})$ space by a deterministic algorithm, where $N$ is the length of the input sequence.
While it is known that deterministic $O(1)$-approximation indeed requires $\Omega(\sqrt{N})$ space, no lower bound results are known that rule out even an $O(1)$ space randomized algorithm for an $O(1)$-approximation of LIS length.
We show that understanding the randomized space complexity of \LIS is closely related to the randomized query complexity of \NCM in the model that we refer to as `hybrid model' and under some natural conditions,  progress on the state-of-the-art for one problem will have significant implications for the other. 

==> ncm/title.tex <==
\title{
    On Streaming Algorithms for Longest Increasing Subsequence and Non-Crossing Matchings in Graphs
} 

\author{
    Julia Chuzhoy\thanks{Toyota Technological Institute at Chicago. Email: {\tt cjulia@ttic.edu}.}
    \and
    Sanjeev Khanna\thanks{Department of Computer and Information Science, University of Pennsylvania. Email: {\tt sanjeev@cis.upenn.edu}.}
    \and Rachit Nimavat\thanks{Toyota Technological Institute at Chicago. Email: {\tt nimavat@ttic.edu}.}
}
\maketitle
